SAFE-RL: Saliency-Aware Counterfactual Explainer for Deep Reinforcement Learning Policies

While Deep Reinforcement Learning (DRL) has emerged as a promising solution for intricate control tasks, the lack of explainability of the learned policies impedes its uptake in safety-critical applications, such as automated driving systems (ADS). Counterfactual (CF) explanations have recently gained prominence for their ability to interpret black-box Deep Learning (DL) models. CF examples are associated with minimal changes in the input, resulting in a complementary output by the DL model. Finding such alternations, particularly for high-dimensional visual inputs, poses significant challenges. Besides, the temporal dependency introduced by the reliance of the DRL agent action on a history of past state observations further complicates the generation of CF examples. To address these challenges, we propose using a saliency map to identify the most influential input pixels across the sequence of past observed states by the agent. Then, we feed this map to a deep generative model, enabling the generation of plausible CFs with constrained modifications centred on the salient regions. We evaluate the effectiveness of our framework in diverse domains, including ADS, Atari Pong, Pacman and space-invaders games, using traditional performance metrics such as validity, proximity and sparsity. Experimental results demonstrate that this framework generates more informative and plausible CFs than the state-of-the-art for a wide range of environments and DRL agents. In order to foster research in this area, we have made our datasets and codes publicly available at https://github.com/Amir-Samadi/SAFE-RL.

==> tex/intro.tex <==

% The necessity of explainability for DRL
%\st{Deep Reinforcement Learning (DRL) has emerged as a powerful decision-making technique in environments with high-dimensional input states where traditional RL algorithms do not perform well}. 
Deep Reinforcement Learning (DRL) has emerged as a powerful decision-making technique for solving intricate control tasks across diverse domains, ranging from robotics~\cite{zhu2021deep} to gaming~\cite{berner2019dota}. This achievement is facilitated by employing Deep Neural Networks (DNNs) that can effectively learn to map high-dimensional state spaces to actions forming the policy of the DRL agent. However, the lack of interpretability in the operation of DNNs and subsequently in the learned policies hinders the application of DRL agents in safety-critical scenarios, such as automated/autonomous driving systems (ADS), where understanding the decision-making process is indispensable~\cite{olson2021counterfactual}. The explicability of the DRL policies becomes paramount, as it fosters trust and empowers human operators to intervene, debug, and ensure transparency of the system's behaviour. As a result, such explanations can aid diverse stakeholders, including end-users, engineers, and legal authorities in understanding the decision-making process that governs the operation of DRL-based systems~\cite{wachter2017counterfactual}. To this end, we investigate counterfactual (CF) explanations, a promising method for eXplainable Artificial Intelligence (XAI) that has recently gained momentum in interpreting the decision-making of black-box DNNs~\cite{samadi2023counterfactual}. A CF explainer entails applying minimal modifications to the input that result in an alternative output from the deep learning model. Comparing the understandable and actionable CF examples with the original state-action pairs can bridge the gap between opaque DRL policies and human-interpretable reasoning.
\begin{figure}
\centering
\includegraphics[width=0.91\linewidth, height=4.1cm]{img/teaser.png}
\vspace{-0.2cm}
\caption{\label{fig: teaser}Overview of the CF generation method for DRL agents. In this illustration, the input and output to the CF explainer consist of four images but only the most recent one is depicted for clarity. While initially, the DRL agent (lock symbolises frozen parameters) decides to accelerate the EGO vehicle (green rectangle) depicted on the left-hand side, the selected action by a user is to slow down the EGO vehicle without performing a lane change. Therefore the SAFE-RL generated a CF state where the EGO vehicle is surrounded by participant vehicles (blue rectangles), depicted on the right-hand side.}
\vspace{-0.4cm}
\end{figure}

Several optimisation methods and deep generative models have been recently utilised for generating CF explanations. Optimisation techniques, including perturbation-based, gradient-based, and genetic algorithms, rely on directly modifying the input data or specific features~\cite{samadi2023counterfactual}. Despite demonstrating promising performances with low-dimensional inputs, such as tabular data, they yield incongruous or adversarial examples when applied to high-dimensional inputs, such as images, which have been extensively studied in the context of adversarial attacks~\cite{goodfellow2014explaining}. Deep generative models, such as Generative Adversarial Network (GAN)~\cite{jacob2022steex, zemni2023octet} and Diffusion Models \cite{jeanneret2022diffusion},  overcome this limitation by synthesising CF inputs instead of altering features in the input. However, these models have not been well-investigated in the context of DRL. %Unfortunately, DRL agents operating with visual states pose extra complexity in CF generation because deep generative models should  process multiple state observations at a time. 

%The ability to make sequential decisions in 
DRL agents, in many applications, process a history of observations at every time step resulting in temporal dependencies in the input that add to the complexity of deep generative models creating CF examples~\cite{huber2023ganterfactual}. 
% The inherent complexity of DRL agents lies in the requirement to make sequential decisions based on a history of observations and actions, resulting in a temporal dependency that adds to the complexity of generating meaningful CF explanations~\cite{huber2023ganterfactual}.
% Unlike supervised learning models, DRL agents perform sequential decisions, where actions are related to previous choices and observations, learning provident policies aimed at delayed rewards~\cite{huber2023ganterfactual}. 
For instance, in Fig.~\ref{fig: teaser}, a DRL-based ADS receives four state observations of the driving environment in each time step (including the current state and the three most recent past states) before taking action. As a result of this dependency, the CF model should generate four high-resolution images (a CF image per state), which extends its complexity. Besides, the generated CF states 
% at each time step, 
(e.g., the four CF state images in Fig.~\ref{fig: teaser}) 
must demonstrate internal consistency, plausibility and a distinct rationale for each complementary action. For instance, in a highway driving scenario, the locations of vehicles in subsequent CF images must represent realistic driving manoeuvres and comply with the speed limits and road geometry. Due to such challenges, to the best of our knowledge, there are merely two available models in the literature that generate CF examples for DRL agents operating with visual data. 

The first, by Olson {\it{et al.}}~\cite{olson2021counterfactual},  relies on a complex combination of DNNs, where a DNN generator model is trained to change the agent's action. However, the user cannot specify the desirable alternate action of the DRL agent, which limits the model's applicability. The second, by Huber {\it{et al.}}~\cite{huber2023ganterfactual}, known as GANterfactual-RL, employs StarGAN~\cite{choi2018stargan}, a well-known image-to-image translation model as the backbone network. Even though both models shed some light on the behaviour of the DRL agents, they often generate implausible or meaningless CFs. This limitation stems from the fact that the applied deep generative models only rely on the state observations without any guidance on how to narrow down the solution space, potentially leading to suboptimal CF solutions in the large visual space domain.
% due to the large space of visual states, that leads to sub-optimal solutions (CF examples). 
Consequently, the existing literature lacks an efficient model capable of generating plausible and meaningful CF examples
 for DRL agents processing visual states. 
% The inherent complexity of DRL agents arises from their ability to make sequential decisions based on previous observations and actions, introducing temporal dependencies that add to the difficulty of generating meaningful CF explanations \cite{huber2023ganterfactual}. For example, the DRL agents used in this study (see Fig. \ref{fig:teaser}) receive four input/state observations to provide an action in each time-step. Consequently, the CF explainer model faces the challenge of generating four modified high-resolution images to produce meaningful CF examples. Despite recent efforts by Olson et al. \cite{olson2021counterfactual} and Huber et al. \cite{huber2023ganterfactual} to propose models for generating CFs in the DRL context, their approaches suffer from generating implausible and less meaningful CFs, partly due to a lack of further guidance to limit the potential solution space.


% This paper introduces a novel framework that employs a Generative Adversarial Network (GAN) to produce CF explanations for RL agents. Our approach leverages saliency maps to pinpoint the most influential pixels for the agent’s output. Saliency maps represent a noteworthy advancement within the domain of XAI, as they offer valuable insights into the focal regions of the input that capture the most attention from the black-box model while making decision  [11]. This breakthrough has the potential to improve the quality of generated Counterfactual (CF) explanations, as it enables selective alterations to be made in sparse regions of the inputs/states. Consequently, this approach allows for the generation of meaningful CF examples. We assess our framework on diverse testbeds spanning automated driving environments and the Atari game Pong. Our experiments validate that the proposed technique generates plausible and informative CF explanations for a wide extent of DRL agent decisions. Nevertheless. To encourage further research, we make our dataset publicly available. The key contributions of this study are summarised in the following list


To bridge the identified gap this paper introduces a novel framework that employs a guided GAN model with saliency maps to produce CF explanations for DRL agents.
% In the context of generating CF explanations for supervised learners, SAFE~\cite{samadi20203SAFE} demonstrated the superiority of corporating saliency maps in CF generation over other translation-to-translation models. This study provides CF explanations specifically designed for DRL agents, by adjusting and reconfiguring the SAFE model architecture, along with proposing novel loss functions to incorporate the use of saliency maps and comprehend the spatiotemporal state observations.
% This is achieved by adapting the SAFE model, which involves reconfiguring and modifying the networks and loss functions. These modifications allow for the integration of saliency maps and a comprehensive understanding of the spatiotemporal state observations.
% The proposed approach builds upon the work by~\cite{samadi20203SAFE} that demonstrated superior CF generation capabilities for supervised learners by incorporating a saliency map into the GAN~\cite{selvaraju2017grad}. 
Saliency maps highlight the most influential input pixels during decision-making, providing valuable insights into the focal regions that capture the most attention from the black-box model. 
% Adapting saliency maps into the DRL domain does not come without cost or challenges. 
In the context of generating CF explanations for supervised learners, we demonstrated, as a preliminary study in~\cite{samadi20203SAFE}, the superiority of incorporating saliency maps in CF generation compared to alternative Image-to-Image translation~(I2I) models. To provide CF explanations for DRL agents, this work improves upon the DNN employed in the deep generative model. Additionally, novel loss functions are proposed to seamlessly integrate the utilisation of saliency maps and to comprehend spatiotemporal state observations.
% we have adjusted the networks used in the SAFE model and proposed novel loss functions to incorporate the use of saliency maps and comprehend the spatiotemporal state observations. 
To encourage further studies in this field, a benchmark is also established, encompassing extensive performance results. Moreover, new datasets are introduced across various environments and DRL agents. In summary, the key contributions of this paper are:    
% Besides computational complexity, the CF images generated at each time step, e.g., the four CF examples in Fig.~\ref{fig:teaser}, must be consistent with each other, plausible and provide a unique explanation for the (complementary) action (selected by the user). For instance, in a highway driving scenario, the locations of vehicles in subsequent CF images must represent realistic driving manoeuvres that exhibit spatiotemporal correlations and comply with the speed limits and road geometry.
% To address those challenges, the key contributions of this paper are: %in the following list:
%Our framework is assessed on diverse test beds spanning ADS  and the Atari game %Pong, demonstrating the generation of plausible and informative CF explanations for a wide range of DRL agent decisions. To encourage further research, we provide new datasets for multiple environments, labeled by three popular DRL agents, including Deep Q-network (DQN)~\cite{mnih2015human}, Asynchronous Actor-Critic (A2C)~\cite{mnih2016asynchronous} and Proximal Policy Optimisation (PPO)~\cite{schulman2017proximal}. 
\begin{enumerate}
    \item 
    The proposition of a novel framework named SAFE-RL, which can be used to interpret DRL agents decisions by integrating a saliency guidance into a GAN for CF generation. 
    %\item Introducing of a novel formulation to fuse the saliency guidance into the DRL-designed GAN, termed SAFE-RL, resulting in the generation of sparse and high-quality CF examples.
    \item The generation of new datasets for multiple environments, including Atari Pong game~\cite{1606.01540}, highway and roundabout driving~\cite{highway-env}, specifically labelled by three popular DRL agents including Deep Q-network (DQN)~\cite{mnih2015human}, Asynchronous Actor-Critic (A2C)~\cite{mnih2016asynchronous} and Proximal Policy Optimisation (PPO)~\cite{schulman2017proximal}. These datasets are made publicly available. %facilitating comprehensive performance analysis and comparisons with baseline methods.
    \item A comprehensive performance evaluation analysis of SAFE-RL in three environments for three DRL agents and demonstration of superior performance in terms of validity, sparsity, and proximity for the generated CF examples as compared to baseline methods by~\cite{olson2021counterfactual} and~\cite{huber2023ganterfactual}. We conduct 27 experiments in total, which can be considered as a benchmark for future studies. The codes for all experiments are  made publicly available. 
\end{enumerate}

Through the above, this paper aspires to improve the explicability of the decision-making process for DRL agents, advance the field of XAI and facilitate the deployment of transparent and trustworthy AI systems in real-world applications, such as ADS. 
% The rest of this paper is organised into the following sections. 

% In summary, the main contributions of this study are as follows:

% This paper introduces a novel framework that leverages a Generative Adversarial Network (GAN) to produce CF explanations for DRL agents. Our approach builds upon the previously published SAFE model, which demonstrated superior CF generation capabilities for supervised learners by incorporating saliency maps \cite{selvaraju2017grad}. By adapting the SAFE model to the DRL domain and utilizing saliency maps, our framework enables the generation of more realistic and interpretable CF examples for DRL agents. We validate our approach on diverse testbeds, including automated driving environments and the Atari game Pong, demonstrating the generation of plausible and informative CF explanations for a wide range of DRL agent decisions. Additionally, we provide new datasets for multiple environments, labeled by triple DRL agents (PPO, DQN, and A2C), to encourage further research in this area.
% Saliency maps represent a noteworthy advancement within the domain of XAI, as they offer valuable insights into the focal regions of the input that capture the most attention from the black-box model while making decisions \cite{selvaraju2017grad}. This breakthrough has the potential to improve the quality of generated Counterfactual (CF) explanations, as it enables selective alterations to be made in sparse regions of the inputs/states. Consequently, this approach allows for the generation of meaningful CF examples. 


% Extending the application of the SAFE model to generate interpretable CF explanations for DRL agents by leveraging saliency maps.
% Introducing a novel formulation to fuse saliency guidance into the DRL-designed GAN, termed SAFE-RL, to produce high-quality CF examples.
% Providing new datasets for multiple environments, facilitating comprehensive performance analysis and comparisons with baseline approaches.
% Demonstrating the superiority of the SAFE-RL framework in terms of validity, sparsity, and proximity of generated CF examples for DRL agents.
% Through these contributions, this paper addresses the pressing need for interpretable explanations in the domain of Deep Reinforcement Learning, bringing us one step closer to achieving transparent and trustworthy AI systems for real-world applications.


==> tex/related.tex <==


%This section presents an overview of the existing research on interpretability in the field of machine learning, with a specific focus on CF explanations. Our emphasis is on deep generative CF methods, which have proved to be very efficient when applied to DL models with visual inputs.
This section presents an overview of the existing research on interpretability in machine learning, focusing on deep generative CF methods, which proved very efficient when applied to DL models operating with high-dimensional visual inputs.
% sub

% \subsection{Interpretability in Deep Learning}

% In recent studies, researchers have explored a variety of techniques aimed at improving the interpretability of DL models, ranging from decision trees~\cite{Zhang_2019_CVPR} to more advanced methods such as sensitivity analysis~\cite{samek2016evaluating}. 
% Interpretability methods in machine learning can be classified into intrinsic and post-hoc models~\cite{chou2022counterfactuals}. Intrinsic methods design and train DNN models that inherently possess interpretability, while post-hoc methods rely on auxiliary models to extract explanations from pre-trained models. Post-hoc explanations are further divided into global, providing a comprehensive view of the main factors influencing the model's decision-making process, and local, aiming to interpret the model's behaviour on specific inputs~\cite{ribeiro2016should}. 

% %This study primarily investigates 
% CF explanation is a subset of post-hoc approaches that offers human-understandable interpretations of the model's behaviour~\cite{wachter2017counterfactual}. Local CF explanations involve minimal modifications to the input data, resulting in the alteration of the model output. 
% They can be used to enhance our comprehension of the factors that influence the decision-making process, e.g., explain why a specific action was chosen and which input features were crucial in that decision.
% For example, in ADS, CF explanations may interpret whether the front or adjacent vehicle behaviour influenced the model's decision to keep or change the lane for the EGO vehicle.
% Traditional CF explanation approaches are based on optimisation methods, including gradient-based techniques~\cite{wachter2017counterfactual} and game theory~\cite{ramon2020comparison}, demonstrating acceptable performance in tabular data~\cite{wachter2017counterfactual}. However, these approaches encounter several difficulties in generating CF examples for DL model that process high-dimensional input data such as high-resolution images. To address this challenge, researchers have proposed deep-generative CF models. 

% sub
% \subsection{Deep Generative CF Explainers}
%One potentially effective method, known as 
To provide explicability for DNNs operating with visual inputs, deep generative models such as GANs have been used to create CF examples, and they are commonly referred to as deep generative CF explainers~\cite{AugustinBC022,jacob2022steex,khorram2022cycle}. 
%Deep generative models for producing CF explanations utilise deep generative models to enhance the comprehensibility of intricate decision-making systems, such as  DNNs~\cite{AugustinBC022,jacob2022steex,khorram2022cycle}. 
One prominent and complicated instance of such models that leverages the latent space of a DRL agent to generate CF images has been proposed by Olson {\it{et al.}} in~\cite{olson2021counterfactual}. GANterfactual-RL is another deep generative CF model that employs starGAN, an I2I model, to provide CF states~\cite{huber2023ganterfactual}. The objective in I2I is to transform an image from one domain to another, e.g., horse to zebra images~\cite{choi2018stargan}. Hence, Huber {\it{et al.}} in~\cite{huber2023ganterfactual} surmised that generating CF explanations resembles a transformation of the input between different domains~(I2I translation). 
% I2I translation for generating CF examples has also been employed for supervised learners~\cite{huber2023ganterfactual}. 
Although such approaches could provide informative CF explanations, generating CFs for DRL agents in complex environments remains challenging, especially when dealing with high-resolution (visual) data and long observation windows.
% This difficulty arises from the need to handle high-resolution (visual) data and long observation horizons. 
Consequently, some studies on CF generations tend to guide the generative models by restricting the potential solutions.  

The use of disentangled latent states is a method for constraining the solution space in the deep-generator model, in which each dimension of the latent state captures a specific characteristic or feature of the generated data. For example, by using a semantic segmentation layer of driving scenes in the STEEX model~\cite{jacob2022steex}, the disentangled latent state contains semantic features of input images, such as traffic lights and participant vehicles information. Zemni {\it{et. al.}} in~\cite{zemni2022octet} leverage object-centered representations of driving scenes to feed a deep generative model that provides object-level CF explanations. 
% Using disentangled latent state enables control and comprehension of the underlying data features that contribute to the CF example generation.
By employing disentangled latent states, it becomes possible to control and comprehend the underlying data features contributing to the CF example generation. 
% The STEEX model~\cite{jacob2022steex}, for example, generates CF examples within driving scenarios from a semantic segmentation layer chosen by the end-user, such as traffic light segmentation. 
% Zemni et al.~\cite{zemni2022octet} leverage a deep generative model objects-centric representation to generate object-aware CF explanations. 
However, it shall be noted that given the alternate action, these CF explanations are derived from a feature space that has been selected by the user, rather than being optimised across the entire input feature space. In our recent study named as SAFE in~\cite{samadi20203SAFE}, we have examined the potential drawbacks of manually selecting input features, which can result in explanations that are suboptimal and biased. However, the SAFE model blindly followed its preceding I2I translation models, resulting in defining inefficient generative models.

In this paper, SAFE-RL introduces substantial enhancements to the generator network to process a sequence of observation states instead of a single image processed in SAFE. This enhancement coupled with revised network layers and loss functions for the generator, have endowed SAFE-RL with spatiotemporal processing capabilities that SAFE lacks. Furthermore, SAFE-RL alleviates the need for the classification objective from its discriminator network, leading to more efficient training and a significant reduction of network parameters by 43\%, as compared to SAFE. Instead, it employs the black-box DRL model for real/fake image classification and introduces a novel loss function in the discriminator. Moreover, SAFE-RL introduces a novel prediction loss for saliency map generation. This change overcomes a limitation in the SAFE model, where the generator simply echoes the self-attention layer's output (Att) for generating CF saliency maps. The introduced prediction loss leads the generator network in SAFE-RL toward more accurate saliency map generation compared to SAFE. \DIFadd{Finally, we found a limitation in the dataset collection algorithm introduced by Huber~{\it et al.}~\cite{huber2023ganterfactual}: it only saved RGB observation states from the current time-step. Consequently, their GAN model could only generate CF states for a single time-step, which were then converted to grayscale and repeated to cover multiple time-steps. This approach risks misleading labels for the DRL agent, affecting the validity of the method, especially in training the discriminator. To overcome this, our proposed dataset collection now includes grayscale observation states from the last four time steps, alongside RGB data for the current time-step. This enhancement enables our deep generator to provide temporal grayscale states in four channels (each representing a previous time step), along with the RGB state for the current time-step. This improvement enhances clarity and precision for end-users and allows for a more accurate evaluation of validity metrics.} In summary, in this research, we reformulated and extended our previous work in~\cite{samadi20203SAFE} for use with a DRL agent explainer.


% In a recent study~\cite{samadi20203SAFE}, Samadi {\it{et al.}}  have examined the potential drawbacks of manually selecting input features, which can result in explanations that are suboptimal and biased. To address this concern, the deep generative CF explainer model named after SAFE gets the DNN's saliency map and applies modifications only in the salient pixels~\cite{samadi20203SAFE}. Inspired by the SAFE model, in this research, we reformulate it for use with a DRL agent explainer, which we hereafter refer to as SAFE-RL.

% Both SAFE~\cite{samadi20203SAFE} and GANterfactual-RL~\cite{huber2023ganterfactual} utilise Image-to-Image Translation models, namely AttentionGAN and StarGAN~\cite{choi2018stargan}, respectively. It is important to note that these models were initially designed without a decision model to classify generated CF images (fake images) into specific classes. As a result, the discriminator model in those methods, follows multiple objectives, including classifying and distinguishing the fake/original images. However, in the context of CF tasks, a black-box model is available to perform this classification. Consequently, we have made significant modifications to the architecture and loss functions of our framework to streamline the model, resulting in notable performance improvements. 

%Inspired by the SAFE model, In this research, we have reformulated the SAFE model for use with a DRL agent explainer, which we refer to as SAFE-RL. To limit the potential solutions and focus on changing relevant regions into the temporal input/state observations, the proposed deep generative model leverages the DRL agent's saliency map. This allows us to generate CF explanations that are more plausible and meaningful in complex environments, where high-resolution visual data and long observation horizons are involved.



%For a given decision model and query input, a CF explanation is defined as a minimally modified version of the query that changes the decision of the model. 
% For instance, in an initial work\cite{liu2019generative}, a trained classifier named as AttGAN provides labels for a cycleGAN~\cite{he2019attgan}. This deep generative model then transfers the input image to the target domain serving as a CF explanation example. In a follow-up work~\cite{huber2023ganterfactual}, a starGAN~\cite{choi2018stargan} is employed to generate CF examples for a  trained reinforcement learning-based model. The authors in~\cite{kothiyalutilization} conducted a comparison of different cycleGAN models for generating CF examples focusing on image quality metrics. The majority of works can explain classifiers working on simple images, such as face portraits or featuring a single and centered object.
% Nevertheless, generating CF explanations in complex environments, such as those encountered in ADS, can be challenging due to the high diversity and scattered distribution of images in the available driving datasets~\cite{jacob2022steex}. To this end, several works tend to limit the solution space for guiding the learning of generative models.

% \st{Initially, counterfactuals were developed for models operating on tabular data \cite{mothilal2020dice}, but they have recently been applied to explain deep computer vision models as well \cite{goyal2019counterfactual,moosavi2016deepfool,vandenhende2022making,jacob2022steex}. One of the challenges is to ensure that the explanations are both minimal and meaningful. Adversarial attacks can be minimal, but they are not informative for the end user \cite{GoodfellowSS14,moosavi2016deepfool}. Retrieval-based methods have been used to mine the dataset for counterfactual explanations, but they can only provide explanations as minimal as the dataset granularity allows \cite{goyal2019counterfactual,hu2022x,vandenhende2022making}.}

% \st{More recently, generator-based counterfactual explanations have been proposed \cite{AugustinBC022,jacob2022steex,khorram2022cycle}. These methods leverage}

% One way to restrict the solution space utilises an encoder-decoder pair in deep generative models, which effectively maps the input data distribution into a disentangled latent space~\cite{jacob2022steex, zemni2022octet}. The latter is a learned feature space where each dimension captures a specific attribute of the data independently of other dimensions, enabling control and understanding of the underlying features of the data that contribute to the generation of the CF example. Deep generative methods can provide minimal and meaningful CF examples by applying optimised manipulations into the latent space. 
% However, such CF explanations are obtained from a user-selected feature space rather than being optimised within the entire input feature space. For instance, the STEEX model in~\cite{jacob2022steex} generates CF examples within the driving environment from a  semantic layer selected by the end-user, such as traffic light segmentation, which might end up being suboptimal as the feature space is restricted. Unlike previous methods, in this study, we use saliency map features which lead the generative model to search near the black-box model's decision boundary, resulting in a global minimum solution. 
%Moreover, STEEX \cite{jacob2022steex} requires annotated semantic segmentation masks of images to work, which is not always available or is costly for the user to produce \cite{zemni2022octet}. Several works have proposed different generator-based approaches to generate CF explanations \cite{kothiyalutilization}. For instance, DIVE \cite{rodriguez2021beyond} exploits the disentangled latent space to generate diverse CF explanations. However, the visual quality of its CFs hinders interpretability. %DVCE  \cite{AugustinBC022} builds on denoising diffusion probabilistic models to achieve better-looking results but lose the more curated control on diversity. 


% \sam{On the other line of work, as an alternative to using disentangled latent state, conditional cycle-GAN methods have been proposed to translate unpaired image-to-image directly. Avoiding intermediate transferring (to the disentangled latent state) enables the deep generative models to extract more comprehensive features (unknown latent state) and decode them to the queried domain. Meanwhile, those extracted features are tied to the given conditional constraints.}

%\st{In the case of complex input data such as perception images collected by ADS, a shift in the input space cannot be expressed by an interpretable mapping function because an interpretable latent space is not known. In practice, conditional cycle-GAN methods have emerged as a solution for unpaired image-to-image translation. They determine the common invariants and changes within a set of CF pairs, effectively explaining the shift from the source to the target distribution. }
% \sam{coppied from the paper: \cite{kulinski2022towards} In some cases, a shift cannot be expressed by an interpretable mapping function because an interpretable latent space is not known. Thus, we can remove the interpretability constraint, and leverage methods from the unpaired Image-to-Image translation (I2I) literature to translate between the source and target domain while preserving the content. For a comprehensive summary of the recent I2I works and methods, please see [14]. Once a mapping is found, to serve as an explanation, we can provide an operator with a set of CF pairs. Then, by determining what commonly stays invariant and what commonly changes across the set of CF pairs, this can serve as an explanation of how the source distribution shifted to the target distribution. While more broadly applicable, this approach could put a higher load on the operator than the interpretable mapping approach.}
%\st{For instance, in an initial work\cite{liu2019generative}, a trained classifier named as AttGAN provides labels for a cycle-GAN, ~\cite{he2019attgan}. This deep generative model then transfers the input image to the target domain, serving as a CF explanation example. In a follow-up work~\cite{huber2023ganterfactual}, a starGAN~\cite{choi2018stargan} is employed to generate CF examples for trained reinforcement learning-based model. The authors in~\cite{kothiyalutilization} conducted a comparison of different cycleGAN models for generating CF examples, focusing on image quality metrics. The majority of works can explain classifiers working on simple images, such as face portraits or featuring a single and centered object. However, scaling up to classifiers operating over more complex images such as crowded urban scenes remains a major challenge.} 

% In this study, avoiding intermediate transferring (to the disentangled latent state) enables our approach to extract more comprehensive features (unknown latent state) and decode them to the queried domain. Meanwhile, for limiting the potential solutions, we use a novel loss function that forces the deep generative model to apply changes merely in salient pixels. Considering that saliency maps encompass decision boundaries~\cite{etmann2019connection, mangla2021saliency}, we have in practice limited the SAcleGAN to apply modifications near the decision boundary regions.

% \sam{we need to select a name for the proposed GAN model, so that mention that name instead of overusing cyleGAN. It also distinguishes our works from those used prepared cyleGAN model only.}\ASh{What about SAcycleGAN (Saliency-aware cycle gan)}


% % past
% {\color{red}

% The field of interpretability is rapidly growing with various research approaches. One approach is post-hoc explanation methods that explain why a model made a specific prediction. These methods can be divided into gradient-based \cite{baehrens2010explain, sundararajan2017axiomatic, smilkov2017smoothgrad, shrikumar2017learning, lundberg2017unified, selvaraju2017grad} that can be reformulated as computing backpropagation for a modified gradient function and perturbation-based approaches \cite{zeiler2014visualizing, suresh2017clinical, ribeiro2016should, tonekaboni2020went} that perturb areas of the input and measure how much this changes the model output. Other approaches aim to measure the reliability of interpretability methods by creating standardized benchmarks \cite{hooker2019benchmark, ismail2020benchmarking, deyoung2020benchmark, tomsett2020sanity, samek2016evaluating,
% petsiuk2018rise} or debugging explanations \cite{ba2014deep, frosst2017distilling, ross2017right, wu2018beyond, ismail2019input}. Some researchers focus on modifying neural architectures for better interpretability. Two previous works \cite{ghaeini2019saliency,ross2017right} incorporate explanations into the learning process but rely on ground truth explanations or annotations, which may not always be available. Our proposed approach does not rely on such annotations and is more practical for datasets with only ground truth labels.
% }
% The problem of generating CF explanations for machine learning models has been the subject of significant research in recent years. In this section, we review some of the related work in the literature.

% One approach to generating CF explanations is through perturbation-based methods. These methods involve systematically perturbing the input data until a CF is found that satisfies certain constraints, such as being close to the original input or adhering to some desired outcome. Examples of perturbation-based methods include the LIME algorithm [1], which generates local linear models to approximate the behavior of the underlying machine learning model, and the CF risk minimization (CRM) method [2], which formulates the CF generation problem as an optimization problem.

% Another approach to generating CF explanations is through gradient-based methods. These methods involve computing gradients with respect to the input data and using them to guide the search for CFs. Examples of gradient-based methods include the influential CF instances (ICI) method [3], which computes gradients with respect to a set of influential instances, and the causal CF learning (CCL) method [4], which uses a causal graph to guide the generation of CFs.

% Recently, several GAN-based methods have also been proposed for generating CF explanations. These methods involve training a GAN to generate CF examples that are similar to the original input but result in a different prediction from the machine learning model. Examples of GAN-based methods include the STEEX method [5], which uses a semantic segmentation network to guide the GAN in generating CFs, and the MAD-GAN method [6], which incorporates a memory module to store past CF examples and encourage diversity in the generated CFs.

% In contrast to the above approaches, our proposed method for generating CF explanations incorporates saliency maps into the CF generator. Saliency maps have been used in previous work for various tasks such as visual attention, object recognition, and image segmentation. By using saliency maps to guide the generation of counterfactual explanations, we aim to generate more interpretable and effective explanations while also reducing the computational cost of the generation process.

% \subsection{saliency generation methods}
% {\color{red}
% five different saliency methods to understand the importance of different input features in determining the output of a model. These methods are:





% Gradient (GRAD) \cite{baehrens2010explain}: This method computes the gradient of the output with respect to the input. It gives a measure of how much each input feature affects the output.

% Integrated Gradients (IG) \cite{sundararajan2017axiomatic}: This method calculates a path integral of the model gradient from a non-informative reference point to the input. It helps to understand the contribution of each input feature in the overall output.

% DeepLIFT (DL)\cite{shrikumar2017learning}: This method compares the activation of each neuron to a reference activation and computes the relevance as the difference between the two activations. It helps to understand the importance of each neuron in determining the output.

% SmoothGrad (SG)\cite{smilkov2017smoothgrad}: This method adds noise to the input and takes the average of the resulting sensitivity maps for each sample. It helps to reduce the noise in the sensitivity maps and get a clearer understanding of the importance of each input feature.

% Gradient SHAP (GS)\cite{lundberg2017unified}: This method adds noise to the input, selects a point along the path between a reference point and the input, and computes the gradient of outputs with respect to those points. It helps to understand the importance of each input feature and how it interacts with other input features.
% }

% \subsection{counterfactual}
% {\color{red}
% }

% \subsection{generative counterfactual}
% {\color{red}

% this paper \cite{huber2023ganterfactual} uses adversarial learning techniques to generate counterfactual explanations for RL agents by formulating the problem as a domain transfer problem, so that they can use starGAN \cite{choi2018stargan}.

% This paper \cite{yang2021generative} proposes a framework called Attribute-Informed Perturbation (AIP) for generating counterfactuals for raw data instances such as text and images. AIP utilizes generative models conditioned with different attributes to obtain counterfactuals with desired labels. The framework optimizes the attribute-informed latent space instead of directly modifying instances in the data space, which improves effectiveness and efficiency. Experimental results demonstrate the effectiveness and sample quality of AIP and its potential for practical applications beyond model interpretability.
% This paper \cite{zhao2020fast} presents a Fast ReAl-time Counterfactual Explanation (FRACE) algorithm that uses Generative Adversarial Networks (GANs) to generate perturbations on a query image that causes it to be classified as a counterfactual. The algorithm uses a residual generator trained on starGAN and a perturbation loss, as well as a classifier, to ensure the generated images are conditional on the classifier and have a minimum change from the query. The FRACE algorithm produces more realistic images compared to previous methods and is faster during inference time. Experimental results show the effectiveness and efficiency of FRACE compared to state-of-the-art methods.
% }
% \subsection{attention guided GAN}
% {\color{red}
% starGAN \cite{choi2018stargan}StarGAN, a scalable approach for image-to-image translation for multiple domains using a single model. This approach leads to superior quality of translated images and the capability to flexibly translate an input image to any desired target domain. StarGAN is demonstrated to be effective on facial attribute transfer and facial expression synthesis tasks.
% AttGAN \cite{he2019attgan} is a framework for high-quality facial attribute editing that uses an attribute classification constraint on the generated image, reconstruction learning, and adversarial learning to ensure visually realistic editing. It outperforms state-of-the-art methods and is extended for unsupervised attribute style manipulation. 
% AttentionGAN \cite{tang2021attentiongan} proposes Attention-Guided Generative Adversarial Networks (AttentionGAN) for the task of unpaired image-to-image translation. The proposed method aims to improve the quality of generated images by identifying the most discriminative foreground objects and minimizing the change of the background. AttentionGAN achieves this by using attention-guided generators that produce attention masks, which are then fused with the generation output to obtain high-quality target images. Additionally, a novel attention-guided discriminator is designed which only considers attended regions. Experimental results on several generative tasks with eight public datasets show that AttentionGAN generates sharper and more realistic images compared to existing competitive models.
% }

% \subsection{generating saliency with GAN}
% {\color{red}
% This paper proposes SalGAN \cite{pan2017salgan}, a data-driven metric based saliency prediction method that uses an adversarial loss function. SalGAN consists of two networks that predict and discriminate saliency maps, respectively. The adversarial training enables SalGAN to achieve state-of-the-art performance across various saliency metrics.

% The authors \cite{sun2020implicit} propose an unsupervised method for extracting implicit saliency in deep neural networks, which performs comparably to state-of-the-art supervised algorithms and is more robust to input noise. The method uses semantic features, lowers the threshold for saliency detection in terms of data, and bridges the gap between human and model saliency.

% This paper \cite{liu2021saliency} proposes a saliency-guided remote sensing image super-resolution method (SG-GAN) that utilizes salient maps to guide the recovery process and focus more on salient objects. Experimental results show that SG-GAN produces competitive results and superior structural restoration compared to advanced methods.
% }
% \subsection{saliency-guided GAN}
% {\color{red}
% This paper \cite{jiang2021saliency} proposes a new task for image-to-image translation, where the translation is conditioned on a user-specified saliency map. The authors propose a Generative Adversarial Network (GAN) called SalG-GAN, which can generate a translated image that satisfies the target saliency map. The model uses a disentangled representation framework to encourage diverse translations for the same target saliency condition. The authors also introduce a saliency-based attention module to help facilitate the structures of the generator, cue encoder, and global and local discriminators. The authors provide a synthetic dataset and a real-world dataset with labeled visual attention to train and evaluate their model. The results of experiments on both datasets show the effectiveness of the proposed model for saliency-guided image translation.


% This paper \cite{sun2023tsrnet} proposes an unsupervised two-stage approach called TsrNet for object-level image style transfer on fashion images. The first stage uses Mask-GAN to identify the clothing texture region, and the second stage utilizes an improved CycleGAN with a Drf-module and GTS to perform texture transfer. The approach is effective and demonstrated through qualitative and quantitative experimental results.
% The paper proposes SGFusion \cite{liu2023sgfusion}, a saliency guided deep-learning framework for pixel-level image fusion. It uses dual-guided encoding, image reconstruction decoding, and saliency detection decoding to extract feature and saliency maps from images. The saliency maps are used as fusion weights to generate the fusion image. SGFusion achieves state-of-the-art performance in different types of image fusion tasks, including infrared and visible image fusion, multi-exposure image fusion, and medical image fusion.

% }
% \subsection{counterfactual using att-GAN}
% {\color{red}
% \cite{liu2019generative} trained classifiers then used attgan\cite{he2019attgan} but they did not used saliency which we did.

% \cite{kothiyalutilization} related works
% The framework described in \cite{singla2023explaining}, generates counterfactual visual explanations for the classifier while using a coditional GAN for transparent decision-making process in healthcare applications. The methodology revolves around perturbation of the original input image such that an explanation function is designed using cGAN keeping in mind the three properties of valid transformation namely: data consistency, classification model consistency and context-aware self-consistency. They used metrics like FID (Frechet Inception Distance), CV (Counterfactual Validity) \cite{mothilal2020explaining} and FOP (Foreign Object Preservation) to support the above three properties for valid transformations. FOP is a metric that they devised which helps in measuring if the patient-specific properties (foreign objects) are retained in the image like pacemaker etc. The intent of the task is similar to our experiment with a difference that in their method, counterfactuals are already images. However, in our experiment the counterfactuals are a human-readable text, that is easier for humans to interpret but difficult for testing and validating. Additionally, their work is specifically for healthcare service line and has been tested on datasets: celebA, MNIST and simulated data in comparison to ours.

% The other model STEEX (STEering counterfactual EXplanations using semantics) implemented in \cite{jacob2022steex} makes use of the latest advancements made in the area of semantic-to-real image synthesis in order to achieve “region-targeted counterfactual explanations” (a concept introduced by the authors), which is the highlight of the paper. Their prime attention is to spotlight the how content-based image classification is vital than only region-based classification which is absolutely true when considering scenarios where safety is of utmost importance like self-driving cars. The metrics used for evaluation in their paper include: FID, Face Verification Accuracy (FVA) and Mean Number of Attributes Changed (MNAC), where the model has been trained for CelebA, CelebAMask-HQ and BDD100k datasets. Similar to the implementation in the previous paper, even this model updates the query image to produce the counterfactual image. Their method involves no textual explanations for producing a counterfactual image which is relatively easier to construe by a human for better understanding as used in our model.

% Another methodology discussed in \cite{goyal2019explaining} talks about Causal Concept Effect (CaCE) measure for interpretability and to get rid of the errors arising from confounding. Their model is based on Variational AutoEncoder (VAE), to estimate VAECaCE metric, which as proposed in the paper can estimate the true concept causal effect. In order to showcase the effectiveness of the CaCE metric, they have tested their model on different datasets like MNIST, COCO Miniplaces and CelebA which clearly exhibits the generalizability of their implemented framework. But however, no GitHub repository links have been shared to support the reproducibility of the code for further research. This paper implements StarGAN for producing the counterfactual images, which is similar to our experiment where we have also used StarGAN to produce counterfactual images for celebA and CUB-200-2011 datasets. However, their experiment does not mention about semantic explanations used for producing counterfactual images but is limited to the causal concept effect.

% PIECE (PlausIble Exceptionality-based Contrastive Explanations) algorithm is one more illustration, which combines a GAN that creates counterfactual and semi-factual explanatory images with a CNN that makes predictions that need to be explained on datasets \cite{kenny2021generating}. This model PIECE uses semantic explanations as a base to generate their counterfactual images just like our model. However, PIECE model has been tested only for datasets: CIFAR-10 and MNIST. Furthermore, Figure 7 from \cite{kenny2021generating} showcases the generated image of a counterfactual explanation for a bird using PIECE and Min-Edit as an image generation model for comparison. It is easily visible to the human eye that the images have a very low resolution, and additionally there is no mention of the resolution of images employed for training the classifier and the counterfactual image generating GAN. Considering the results showcased in the paper, their model PIECE performs better in comparison to other methods like Min-Edit, C-Min-Edit, Proto-CF (Interpretable Counterfactual Explanations Guided by Prototypes) and CEM (Contrastive Explanations Method) for the five metrics presented in Table 1 of the report and scores low only for the optimization time taken for each image, which as per the authors can be compensated by utilizing a GPU or reducing the number of epochs.


% As it is clear from the above-mentioned models that research in this specific domain of adding interpretability to counterfactuals is either limited to a specific domain like healthcare or have been tested on simpler datasets like CelebA, MNIST, CIFAR etc. Therefore, we had to take a step further while implementing our model by parsing the complex dataset of CUB-200-2011, which contains 312 attributes for each bird with a total collection of 11,788 images belonging to 200 class labels. Additionally, we needed latest metrics which could measure the feature vector distance in the images and also indicate their perceptual similarity like FID and LPIPS scores.

% In this paper \cite{kang2022fair}, the authors propose a method to address concerns about racial and gender disparities in facial attribute classification by generating synthetic images that consider both factual and counterfactual assumptions about sensitive attributes. This is done using a causal graph-based approach with an encoder-decoder framework, and the attribute classifier is trained using counterfactual regularization. The proposed method is different from previous works, as it uses a causal graph to generate counterfactual images that preserve the identity of the given image. The approach is tested on the CelebA dataset and shows effectiveness and interpretability in classifying multiple face attributes.
% }
% \subsection{counterfactual using sal-GAN}
% {\color{red}
% }
